Diba: A Re-configurable Stream Processor

Stream processing acceleration is driven by the continuously increasing volume and velocity of data generated on the Web and the limitations of storage, computation, and power consumption. Hardware solutions provide better performance and power consumption, but they are hindered by the high research and development costs and the long time to market. In this work, we propose our re-configurable stream processor (Diba), a complete rethinking of a previously proposed customized and flexible query processor that targets real-time stream processing. Diba uses a unidirectional dataflow not dedicated to any specific type of query (operator) on streams, allowing a straightforward placement of processing components on a general data path that facilitates query mapping. In Diba, the concepts of the distribution network and processing components are implemented as two separate entities connected using generic interfaces. This approach allows the adoption of a versatile architecture for a family of queries rather than forcing a rigid chain of processing components to implement such queries. Our experimental evaluations of representative queries from TPC-H yielded processing times of 300, 1220, and 3520 milliseconds for data streams with scale factor sizes of one, four, and ten gigabytes, respectively.

==> query_assignment.tex <==
\subsection{TPC-H Third Query Prototype}\label{sec:query_assignment}

To evaluate the functionality and properties of our \newfqp, we present an
in-depth description of the query mapping (to the processing blocks) and the
programming steps to realize the TPC-H third (shipping priority) query. This
query retrieves the shipping priority and potential revenue, defined as the
$sum\ of\ l\_extendedprice \times (1-l\_discount)$, of the orders having the
largest revenue among those that had not been shipped as of a given date. Orders
are listed in decreasing order of revenue. If more than 10 unshipped
orders exist, only the 10 orders with the largest revenue are listed. Further details are available in the TPC-H benchmark$^{TM}$ standard specification
manual~\cite{Council08_TPC-H}.

\subsubsection{TPC-H Query Modification} 

To execute the third query on our \newfqp, we need to change the concept of
tables to sliding windows and feed each row in a table as a tuple to our stream
processing engine. In queries with stateful operators, various sliding window
sizes and the order of the reception of new tuples with respect to streams'
origins affect the results. This is a property of stream processing engines and
needs to be accounted for in realistic use cases. Therefore, considering the
effects of these factors is beyond the scope of this work.

To feed the rows of tables as tuples to \newfqp\, we allocate a sufficient
number of bits per each field used in the processing. In
Figure~\ref{fig:streams_to_bits}, we observe the mapping of the third query
table's attributes into different fields, where each attribute field is
specified by a number of bits. Subsequently, the total width of a tuple for each
stream is calculated by the sum of its fields' bits.

\subsubsection{Query Assignment}

The choice of the \newfqp\ topology is flexible and can be decided depending on
the system requirements. In the following, we present an example of the TPC-H
third query assignment to a \newfqp\ instance that is drawn in detail in
Figure~\ref{fig:q3_mapping}. The assigned components are color coded to
demonstrate the mapping between the VHDL realization and the \newfqp\ topology.

The \newfqp\ instance for this example has four topology bricks that are
arranged in four rows and one column. Note that there is no limitation on the
size and form of the chosen topology. In Figure~\ref{fig:q3_mapping}a, the
indexing values defined by ROW and COLUMN refer to each topology brick. For
example, the first brick contains a bypass unit, a selection (Q3\_SEL1) on the
lineitem stream (built from its equivalent table), a selection (Q3\_SEL2) on the
customer stream, and a selection (Q3\_SEL3) on the orders stream.

A bypass unit is a pass-through without any internal components, and having one
of these units in each topology brick is necessary to transfer instructions to
the next row brick. The existence of the bypass unit prevents additional
complications in the logic of other processing units by offloading the unrelated
task of bypassing streams and instructions. Therefore, a topology brick can
contain at least two units, while the upper limit is defined by the application
requirements and fan-out limitations of the chosen hardware.

The TOPO\_MATRIX\-\_INSTANCE realization in VHDL, Figure~\ref{fig:q3_mapping}a,
contains the identifiers of processing units that are instantiated later using
the VHDL GENERATE construct, as shown in Figure~\ref{fig:q3_mapping}b. As an
example, the C\_TPCH\-\_Q3\_C\-M\-JOIN\_Inst hardware unit is instantiated and
connected to the remaining components since its identifier (Q3\_\-CMJOIN) exists
in Figure~\ref{fig:q3_mapping}a.

\begin{figure}[t]
	\centering
	\begin{subfigure}[t]{0.8\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/q3_cmjoin1}
		\caption{Direct assignment}
		\label{fig:q3_cmjoin1}
	\end{subfigure}
	
	\begin{subfigure}[t]{0.8\linewidth}
		\centering
		\includegraphics[width=1\linewidth]{figures/q3_cmjoin2}
		\caption{Optimized}
		\label{fig:q3_cmjoin2}
	\end{subfigure}
	\vspace{-3mm}
	\caption{\cmj\ architecture customized for TPC-H 3rd query.}
\end{figure}

From each tuple, only the necessary fields are fed into hardware to avoid
transmitting/handling unnecessary data. This part inherently implements the
projection operation as one of the tasks of the decomposer component (presented
in Figure~\ref{fig:fqpv2completesystem}) in the complete system. The remaining
operators are placed in the \newfqp\ instance, as shown in
Figure~\ref{fig:q3_mapping}c, with the exception of the aggregation and groupby
operators, which are merged together in one unit, namely, Q3\_G\-ROUPBY\_AGG, in
Figure~\ref{fig:q3_mapping}a.

To simplify the representation, we show the communication network (\scnoc)
separate from the \newfqp\ processing units in Figure~\ref{fig:q3_mapping}d. The
respective instructions for the programming of the \scnoc for the TPC-H third
query are shown in Figure~\ref{fig:q3_mapping}e. These instructions are fed into
the \newfqp\ hardware one-by-one to define the streams' path in each \gs\ and
\ls. In addition to the third query streams, we define an extra stream that only
contains one tuple to indicate the end of streams, referred to as END\_MESSAGE.
The end tuple is fed into the \newfqp\ hardware after the end of all streams.
This tuple's existence is necessary for the groupby and orderby operators to
notify them of the end of operations, correspondingly pushing the resulting data
from them.

\subsubsection{Multiway Hash-based Stream Joins}

We utilize our hash-based join in a custom 3-way stream join for the third query
to show the potential throughput while making it possible to execute TPC-H
benchmarks in reasonable time. Using our hash-based approach, we need to
replicate the \textit{orders} stream stage, once indexed based on the o\_custkey
field and once indexed based on the o\_orderkey field. The resulting
architecture, the customized version of \cmj\ (Figure~\ref{fig:scale_msjoin}),
is shown in Figure~\ref{fig:q3_cmjoin1}. Note that due to the simplification of
the multiway stream join operator in the third query, we do not need the
circular path, which is shown by a disconnection mark in this figure. Since each
incoming tuple is processed in at most one of the indexed sliding windows (either
o\_custkey or o\_orderkey), we can further optimize the design by placing both of
the order stream indexed stages into one stage to improve the efficiency of the
system, which leads to the architecture shown in Figure~\ref{fig:q3_cmjoin2}.

In Figure~\ref{fig:q3_cmjoin2}, each new tuple is stored in its corresponding
sliding window. For processing of the orders stream, tuples start their
execution at the customer stage, and the resulting tuples are emitted from the
lineitem stage. The customer stream tuples start their execution at the orders
stage, and the intermediate results of this stage pass through, without
processing, the customer stage, and the final results are output from the
lineitem stage. Finally, the lineitem stream tuples start their processing at
the orders stage, and the resulting tuples are emitted from the customer stage.
